Explaining the extended GeV gamma-ray emission adjacent to HESS J1825-137

HESS J1825-137 is one of the most powerful and luminous TeV gamma-ray pulsar wind nebulae (PWN). To the south of HESS J1825-137, Fermi-LAT observation revealed a new region of GeV gamma-ray emission with three apparent peaks (termed here, GeV-ABC). This study presents interstellar medium (ISM) data and spectral energy distribution (SED) modelling towards the GeV emission to understand the underlying particle acceleration. We considered several particle accelerator scenarios - the PWN associated with HESS J1825-137, the progenitor SNR also associated with HESS J1825-137, plus the gamma-ray binary system LS\,5039. It was found that the progenitor SNR of HESS J1825-137 has insufficient energetics to account for all GeV emission. GeV-ABC may be a reflection of an earlier epoch in the history of the PWN associated with HESS\,1825-137, assuming fast diffusion perhaps including advection. LS\,5039 cannot meet the required energetics to be the source of particle acceleration. A combination of HESS J1825-137 and LS 5039 could be plausible sources.

==> alternate_discussion.tex <==

\subsection{Accelerator related to \HESSsource} \label{sec:1825_discussion}

\subsubsection{A progenitor SNR}
% \par %new paragraph
% Around $10-30\%$ of the kinetic energy released by a supernova ($10^{51}~\ergs$) is channelled into acceleration of high energy particles (with $1\%$ of this energy being funnelled into electrons). A basic assumption that can be made is that the release of these cosmic rays are isotropic. In reality it can be observed in Fig.\,\ref{fig:CO_data} and Fig.\,\ref{fig:HI_data} that relatively dense gas lies to the north. Similarly, H$\alpha$ clouds lie to the north of \HESSsource assuming that these clouds, as seen in Fig.\,\ref{fig:H_alpha}, lie at the same distance as \HESSsource.  This dense gas will slow the propagation of cosmic rays to the north removing the symmetry of particle escape.
\par %new paragraph
The progenitor SNR linked to \HESSsource is an example of an impulsive accelerator; releasing approximately $10^{50}~\ergs$ of cosmic rays (including electrons). As the system evolves, the SNR expands and cosmic rays will escape from the system, decreasing the total energy of particles trapped inside the SNR. From spectral energy distribution modelling, the energy budget in region GeV-A, GeV-B and GeV-C required to reproduce the SED is obtained. This is reflected in Table\,\ref{tab:SED_sum_1825} as $W$. Using the above assumptions, the total SNR cosmic ray energy budget, $W_\text{SNR}$, can be estimated by equation \ref{eq:filling_factor}. This can be seen in the final column of Table\,\ref{tab:SED_sum_1825}. 
\par %new paragraph
To reproduce the SED of any of GeV-A, B \& C requires a pure impulsive leptonic energy budget of, at least,  $10^{50}~\ergs$ within the SNR, as shown in Table\,\ref{tab:SED_sum_1825}. As discussed previously, around $10^{48}~\ergs$ of energy is channeled into electrons. An impulsive leptonic model of \HESSsource for ages of $21.4~\kiloyear$ and $40~\kiloyear$ requires total electron energy budgets of $7.3\times 10^{50}~\ergs$ and $9.4\times 10^{50}~\ergs$ respectively. Therefore an impulsive leptonic model of \HESSsource being the accelerator of high energy particles resulting in the $GeV$ gamma-radiation as observed by \fermi-LAT is rejected. Similarly a hadronic impulsive model cannot simultaneously explain the gamma-ray emission from GeV-A, B \& C. It can be observed in Table\,\ref{tab:total_density} that the hydrogen density is not constant across GeV-A, B \& C..Eq.\,\ref{eq:app_proton_proton_flux} shows that the spectra of gamma-rays from proton-proton interactions is proportional to the density of the target material. If the high density cloud observed in the $15-30~\kmpersec$ range lies at the same distance as \HESSsource then GeV-B should appear brighter in gamma-rays compared to GeV-A and GeV-C assuming that the cosmic ray energy density over all three regions are constant. As this is not the case, if a hadronic scenario is the source, the cosmic ray energy density in cloud A \& C must be roughly $7$ \& $80$ times greater respectively than the energy density in cloud B. Unless there is energy dependent ISM interactions, there is no reason why the cosmic ray energy density in cloud A \& C is greater than in cloud B; disfavouring an impulsive hadronic scenario. If the high density cloud observed in the $15-30~\kmpersec$ is in the foreground of HESS\,J1825-137, this will increase the energy budget required to reproduce the SED roughly by an order of ten as shown in Table\,\ref{tab:SED_sum_1825}. In this scenario the SNR must contain $\approx 10^{51}~\ergs$ of cosmic rays for system age of $21~\kiloyear$ and $40~\kiloyear$.
\par %new paragraph
A leptonic-hadronic impulsive scenario requires leptonic interactions to produce $1\%$ of the GeV gamma-rays as seen by \fermi-LAT to reduce the total SNR leptonic energy budget to $10^{48}~\ergs$. This leaves $99\%$ of gamma-rays from GeV-A, B \& C to be the result of proton-proton interactions from SNR with hadronic energy budget of $\approx 10^{51}~\ergs$. Therefore an impulsive scenario considering a combination of hadronic \& leptonic interactions forming the observed GeV gamma-rays can be rejected.
\par %new paragraphs
An impulsive scenario where the supernova related to \HESSsource is the only source of cosmic rays (leptonic and hadronic) that produce the GeV gamma-ray emission as observed by \citep{Araya:2019dez} can be rejected.

\subsubsection{PWN}
We will now discuss the possibility of the PWN powered scenario as the accelerator for high energy particles.
\par %new paragraph
The spin down power of the pulsar powering PWN \HESSsource is of order $10^{36}~\ergspersecond$. The spin down power of the pulsar is not constant over time; \citep{2006A&A...460..365A} has suggested that the high gamma-ray luminosity may indicate that the spin down power was far greater in the fast. The luminosity of x-rays between $0.5-10~\keV$ is around $3\times 10^{33}~\ergspersecond$ \citep{2006A&A...460..365A}; compared to the luminosity in gamma rays above $300~\GeV$ \citep{2019A&A...621A.116H}. 
\par %new paragraph
From Table\,\ref{tab:SED_sum_1825} a continuous hadronic scenario for both ages requires at least $10^{37}~\ergspersecond$ to be channelled into protons, rejecting this scenario. 
Considering a leptonic continuous scenario for ages of $21~\kiloyear$ and $40~\kiloyear$, all three GeV regions require a total of $\approx 10^{37}~\ergspersecond$ in injection luminosity. This is even higher for a hadronic continuous scenario; requiring injection luminosities of $1.8\times 10^{39}~\ergspersecond$ \& $9.4\times 10^{38}~\ergspersecond$ for ages $21~\kiloyear$ and $40~\kiloyear$ respectively.
% Considering a leptonic continuous scenario; if the pulsar is $21~\kiloyear$ old, then all three objects require of order $10^{37}~\ergspersecond$ of energy to power the GeV emission. PSR\,J1826-1334 is unable to provide this kind of energy. This is still the case if the system towards \HESSsource was $40~\kiloyear$ old rather than $21~\kiloyear$. Although the energy required for objects GeV-B \& GeV-C decreases to order $10^{36}~\ergs$, but this energy budget reflects the energy required to produce GeV emission from GeV-B \& GeV-C individually, not the combined energy budget from GeV-ABC. Even if all the spin down power of the pulsar is converted into high energy particles, not all this energy is channelled into GeV-ABC. Therefore an older leptonic continuous scenario is also disfavoured even if considering the particle transport towards GeV-ABC as noted by \citep{2019A&A...621A.116H}.
\par %new paragraph
In summary it can be concluded from SED modelling that a PWN process powering new region of GeV gamma-ray emission can be rejected.

\subsubsection{Particle Transport between PWN and GeV-ABC}

Fig.\,\ref{fig:Particle_Transport} shows diffusive particle transport of electrons travelling a distance of $70~\pc$ in ambient density of $n=1~\centimeterminusthree$ versus the cooling of synchrotron and IC processes. This is equivalent to the distance that electrons travel after being emitted by the pulsar to reach GeV-B. As shown by the intersection of diffusive transport (assuming $\chi=0.1$) and age of PWN in Fig.\,\ref{fig:Particle_Transport}, electrons with energy $>10~\TeV$ are allowed to reach GeV-B from the PWN before all energy is lost to synchrotron processes. This is reaching the cutoff energy required to reproduce spectral energy distribution of all leptonic process as seen in Table.\,\ref{tab:SED_sum_1825}. A smaller value of $\chi=0.01$ increases the minimum electron energy reaching GeV up to $10^2~\TeV$.
\par %new paragraph
A more powerful pulsar can convert more of its spin down power into electron energy, allowing a greater proportion of higher energy electrons. In turn this allows more electrons to reach GeV-ABC in time to emit $\GeV$ radiation. Therefore unless advection or fast diffusion is considered or the PWN is powerful, electrons are unable to reach GeV-ABC from PSR\,J1826-1334 without significant energy losses.
\par % new paragraph
In IC processes, the final energy of the photon, $E_{\Gamma, \TeV}$, is related to initial electron energy, $E_{e,\TeV}$ and initial photon energy $E_{i,\eV}$ through:


\begin{align}
    E_{\Gamma,\TeV}&=E_{e,\TeV} \frac{2.1b}{\qty(1+(2.1b)^{0.8})^{1/0.8}}
\end{align}

where $b\approx 15E_{\TeV}E_{i,\eV}$ \citep{2009ARA&A..47..523H}. Photons up to $54~\TeV$ has been observed towards \HESSsource \citep{2019A&A...621A.116H}. Assuming IC interactions with the cosmic microwave background are responsible for this emission, this is equivalent to an electron with maximum energy of $96~\TeV$. As shown by Fig\,\ref{fig:Particle_Transport}: possible electrons with energies below $96~\TeV$ is shown to the left of the vertical line. This further limits how many electrons are able to diffuse to GeV-B.
% As shown by Fig\,\ref{fig:Particle_Transport} this further limits how many electrons are able to diffuse to GeV-B.

\subsection{LS5039}

\subsubsection{Progenitor SNR}

From Table\,\ref{tab:SED_sum_5039}, if GeV-ABC is the result of hadronic interactions from an impulsive progenitor SNR, no age of LS\,5039 can simultaneously explain the $\GeV$ emission. Due to the denser cloud towards GeV-B as seen in Fig.\,\ref{fig:CO_data} fo;r all three clouds to be explained by the same source of high energy particles, the cosmic ray density must be approximately a factor of $10$ larger in GeV-B than GeV-A \& GeV-C. It can be concluded that an impulsive hadronic source of cosmic rays from LS\,5039 cannot simultaneously explain the $\GeV$ regions observed by \cite{Araya:2019dez}. Similarly an impulsive leptonic source for any age cannot explain any of the $\GeV$ emission from GeV-ABC.
% The distance between LS\,5039 and GeV- B, assuming both lie in plane $2.5~\kpc$ away, is approximately $45~\pc$.

\subsubsection{Accretion powered}

At an age of $10^3~\si{yr}$, the minimum luminosity energy, for a hadronic scenario, to replicate the GeV gamma-ray emission is of order $10^{38}~\ergspersecond$. This is far greater than the accretion luminosity of LS\,5039. A leptonic model is also not favoured at an age of $10^3~\si{yr}$ with a minimun luminosity energy of $10^{37}~\ergspersecond$. Therefore if \mbox{LS 5039} is the source of the new region of gamma-ray activity, it is unlikely to be a young age.
\par %new paragraph
If LS\,5039 has an age of $10^{5}~\si{yr}$, which is most likely \citep{2012A&A...543A..26M}, a hadronic scenario is still disfavoured with GeV-B having an energy budget of $2.0\times 10^{36}~\ergspersecond$. Even if this energy is still plausible, the cosmic ray energy density of GeV-A \& GeV-C needs to be a factor of 10 greater than GeV-B to produce the same amount of gamma-rays. A leptonic model is far more promising but still unlikely with GeV-ABC requiring combined energy budget of $1.5\times 10^{36}~\ergspersecond$. This does require a harder electron spectra compared to a younger age of LS\,5039 for clouds A \& C with $\Gamma = 1.7$ \& $1.5$ respectively.
\par %new paragraph
At the maximum age of $10^6~\si{yr}$, a hadronic model for LS\,5039 is still unlikely as GeV-C alone requires an energy budget of $2.0\times 10^{36}~\ergspersecond$. A leptonic model is favoured at an age of $10^6~\si{yr}$ with the maximum energy budget needed to reproduce the spectral energy distribution of GeV-ABC is $1.0\times 10^{36}~\ergspersecond$. The energy budget/injection luminosity in Table\,\ref{tab:SED_sum_5039} can vary up to $56\%$, bring the maximum energy budget close to the $5.3\times 10^{35}~\ergspersecond$ injection luminosity partitioned into GeV-ABC. A decrease of injection luminosity as the age of LS\,5039 increases is to be expected; as the system ages, more particles are released resulting in an increase in the spectral energy distribution. Eventually the system reaches a steady state.
\par %new paragraph
Using calculated hydrogen densities towards the regions of interest in LS\,5039 in the $40-60~\kmpersec$ range rather than the $15-30~\kmpersec$ range will not alter the results due to values being with a factor of 10 of each other.
\par %new paragraph
LS\,5039 may be a possible source of the new region of GeV gamma-ray emission assuming that the relativistic jet contains electrons and the age of the system is greater than $10^5~\si{yrs}$. While the jet generally points in the direction of GeV-B (see \ramiref), the precession of the jet may allow electrons to be channeled into GeV-A and GeV-C. Particles may also diffuse from the jet escaping into the necessary regions.

==> old_table.tex <==
\begin{table*}
    \begin{threeparttable}
    \caption{SED model parameters matching the observed emission of GeV-A, B or C. The particle accelerators considered are the impulsive progenitor SNR emission of high energy particles associated with \HESSsource or the subsequent continuous injection of particles by the PWN. High energy particles are assumed to be injected with a power law spectra: $\dv{N}{E} \propto E^{-\Gamma}\exp\qty[E/E_c]$.}
	\centering
	\begin{tabular}{c|cccccccc}
		\hline
		 Accelerator & \multicolumn{8}{c}{\rule{2cm}{0.5pt} Hadronic \rule{2cm}{0.5pt}}\\
		 \HESSsource & Object & $n_H$ ($\centimeterminusthree$) & $W$\footnote{1} or $\dot{W}$\footnote{2} & & $\Gamma$ & $E_C$ ($\TeV$) & $W_\text{SNR}$\footnote{3} or $\dot{W}_\text{tot}$\footnote{4}  & \\
		 \hline
		 Impulsive (SNR) & A & $14$ & $1.0\times 10^{50}$ & $\ergs$ & $2.0$ & $50$ & $6.0\times 10^{51}$ & $\ergs$ \\
		$t=21\times 10^3~\si{yrs}$ & \textbf{B} & $\boldsymbol{79.8}$ & $\boldsymbol{1.5\times 10^{49}}$ & & $\boldsymbol{2.0}$ & $\boldsymbol{50}$ & $\boldsymbol{4.7\times 10^{50}}$ & \\
		 & B & $7.0$ & $1.5\times 10^{50}$ & & $2.0$ & $50$ & $4.7\times 10^{51}$ & \\
		 & C & $1.0$ & $1.2\times 10^{51}$ & & $2.0$ & $50$ & $7.3\times 10^{52}$ & \\
		 \hline
		 Impulsive (SNR) & A & $14$ & $1.0\times 10^{50}$ & $\ergs$ & $2.0$ & $50$ & $6.1\times 10^{51}$ & $\ergs$ \\
		$t=40\times 10^3~\si{yrs}$ & \textbf{B} & $\boldsymbol{79.8}$ & $\boldsymbol{1.5\times 10^{49}}$ & & $\boldsymbol{2.0}$ & $\boldsymbol{50}$ & $\boldsymbol{4.7\times 10^{50}}$ & \\
		 & B & $7.0$ & $1.5\times 10^{50}$ & & $2.0$ & $50$ & $4.7\times 10^{51}$ & \\
		 & C & $1.0$ & $1.1\times 10^{51}$ & & $2.0$ & $50$ & $6.7\times 10^{52}$ & \\
		 \hline
		Continuous (PWN) & A & $14$ & $1.2\times 10^{38}$ & $\ergspersecond$ & $2.0$ & $50$ &  & \\
		$t=21\times 10^3~\si{yrs}$ & B & $79.8$ & $2.0\times 10^{37}$ & & $2.0$ & $50$ &  & \\
		 & B & $7.0$ & $2.2\times 10^{38}$ & & $2.0$ & $50$ &  & \\
		 & C & $1.0$ & $1.7\times 10^{39}$ & & $2.0$ & $50$ & $1.8-2.0\times10^{39}$ & $\ergspersecond$ \\
		 \hline
		Continuous (PWN) & A & $14$ & $8.0\times 10^{37}$ & $\ergspersecond$ & $2.0$ & $50$ & &  \\
		$t=40\times 10^3~\si{yrs}$ & B & $79.8$ & $1.25\times 10^{37}$ & & $2.0$ & $50$ & & \\
		 & B & $7.0$ & $1.25\times 10^{38}$ & & $2.0$ & $50$ & & \\
		 & C & $1.0$ & $8.5\times 10^{38}$ & & $2.0$ & $50$ & $0.9-1.0\times 10^{39}$ & $\ergspersecond$ \\
		\hline
		\hline
		Accelerator & \multicolumn{8}{c}{\rule{2cm}{0.5pt} Leptonic \rule{2cm}{0.5pt}}\\
		 \HESSsource & Object & $n_H$ ($\centimeterminusthree$) & $W$ or $\dot{W}$ & & $\Gamma$ & $E_C$ ($\TeV$) & $W_\text{SNR}$ or $\dot{W}_\text{tot}$ & \\
		 \hline
		 Impulsive (SNR) & A & $14$ & $1.2\times 10^{49}$ & $\ergs$ & $2.0$ & $10$ & $7.3\times 10^{50}$ & $\ergs$ \\
		$t=21\times 10^3~\si{yrs}$ & B & $79.8$ & $9.0\times 10^{48}$ & & $2.0$ & $30$ & $2.8\times 10^{50}$ & \\
		 & B & $7.0$ & $8.0\times 10^{48}$ & & $2.0$ & $30$ & $2.5\times 10^{50}$ & \\
		 & C & $1.0$ & $7.0\times 10^{48}$ & & $2.0$ & $10$ & $4.3\times 10^{50}$ & \\
		 \hline
		 Impulsive (SNR) & A & $14$ & $1.4\times 10^{49}$ & $\ergs$ & $2.0$ & $10$ & $8.5\times 10^{50}$ & $\ergs$ \\
		$t=40\times 10^3~\si{yrs}$ & B & $79.8$ & $6.0\times 10^{48}$ & & $1.0$ & $50$ & $1.9\times 10^{50}$ & \\
		 & B & $7.0$ & $3.0\times 10^{48}$ & & $1.5$ & $50$ & $9.4\times 10^{49}$ & \\
		 & C & $1.0$ & $7.6\times 10^{48}$ & & $2.0$ & $50$ & $4.6\times 10^{50}$ & \\
		 \hline
		 Continuous (PWN) & \textbf{A} & $\boldsymbol{14}$ & $\boldsymbol{1.5\times 10^{37}}$ & $\ergspersecond$ & $\boldsymbol{2.0}$ & $\boldsymbol{10}$ &  &  \\
		$t=21\times 10^3~\si{yrs}$ & \textbf{B} & $\boldsymbol{79.8}$ & $\boldsymbol{1.5\times 10^{37}}$ & & $\boldsymbol{2.0}$ & $\boldsymbol{10}$ &  & \\
		 & \textbf{B} & $\boldsymbol{7.0}$ & $\boldsymbol{1.5\times 10^{37}}$ & & $\boldsymbol{2.0}$ & $\boldsymbol{10}$ &  & \\
		 & \textbf{C} & $\boldsymbol{1.0}$ & $\boldsymbol{1.0\times 10^{37}}$ & & $\boldsymbol{2.0}$ & $\boldsymbol{10}$ & $\boldsymbol{4.0\times 10^{37}}$  & $\ergspersecond$ \\
		 \hline
		Continuous (PWN) & \textbf{A} & $\boldsymbol{14}$ & $\boldsymbol{1.0\times 10^{37}}$ & $\ergspersecond$ & $\boldsymbol{2.0}$ & $\boldsymbol{10}$ &  &  \\
		$t=40\times 10^3~\si{yrs}$ & \textbf{B} & $\boldsymbol{79.8}$ & $\boldsymbol{2.6\times 10^{36}}$ & & $\boldsymbol{1.7}$ & $\boldsymbol{10}$ &  & \\
		 & \textbf{B} & $\boldsymbol{7.0}$ & $\boldsymbol{1.6\times 10^{36}}$ & & $\boldsymbol{1.7}$ & $\boldsymbol{10}$ &  & \\
		 & \textbf{C} & $\boldsymbol{1.0}$ & $\boldsymbol{6.0\times 10^{36}}$ & & $\boldsymbol{2.0}$ & $\boldsymbol{10}$ & $\boldsymbol{1.8-1.9\times 10^{37}}$ & $\ergspersecond$ \\
		 \hline
% 		Continuous (PWN) & A & $14$ & $1.5\times 10^{37}$ & $\ergspersecond$ & $2.0$ & $10$ &  &  \\
% 		$t=21\times 10^3~\si{yrs}$ & B & $79.8$ & $1.5\times 10^{37}$ & & $2.0$ & $10$ &  & \\
% 		 & B & $7.0$ & $1.5\times 10^{37}$ & & $2.0$ & $10$ &  & \\
% 		 & C & $1.0$ & $1.0\times 10^{37}$ & & $2.0$ & $10$ & $4.0\times 10^{37}$  & $\ergspersecond$ \\
% 		 \hline
% 		Continuous (PWN) & A & $14$ & $1.0\times 10^{37}$ & $\ergspersecond$ & $2.0$ & $10$ &  &  \\
% 		$t=40\times 10^3~\si{yrs}$ & B & $79.8$ & $2.6\times 10^{36}$ & & $1.7$ & $10$ &  & \\
% 		 & B & $7.0$ & $1.6\times 10^{36}$ & & $1.7$ & $10$ &  & \\
% 		 & C & $1.0$ & $6.0\times 10^{36}$ & & $2.0$ & $10$ & $1.8-1.9\times 10^{37}$ & $\ergspersecond$ \\
% 		 \hline
	\end{tabular}
	\begin{tablenotes}
	\item \footnotemark[1]{$W$: Energy budget of high energy particles within individual clouds (see Fig. \ref{fig:CO_data})} 
    \item \footnotemark[2]{$\dot{W}$: Particle injection luminosity of high energy particles into individual clouds} 
    \item \footnotemark[3]{$W_\text{SNR}$: Injected energy budget of high energy particles within progenitor SNR (see equation \ref{eq:filling_factor})} 
	\item \footnotemark[4]{$\dot{W}_\text{tot}$: Total injection luminosity of all three regions by PWN}
    \item Plausible scenarios are shown in bold
    \item Matching scenarios have have systematic variation of up to $56\%$ in energy budget $W$ or luminosity $\dot{W}$, $12\%$ in the spectral index $\Gamma$ and $12\%$ in the cutoff energy $E_c$ (see text and figure \ref{fig:example_SED})
    \end{tablenotes}
	\label{tab:SED_sum_1825}
	\end{threeparttable}
\end{table*}

\begin{table*}
    \begin{threeparttable}
    \caption{Model parameters matching the observed emission of GeV-A, B or C. The particle accelerators considered are the progenitor SNR associated with LS\,5039 (impulsive) or the accretion of matter by the companion star onto LS\,5039 (continuous). Example SED best fit is shown in Fig.\,\ref{fig:example_SED}. $W$ or $\dot{W}$ represents the energy budget. To see the regions used, refer to Fig.\,\ref{fig:HI_data}. The spectra of injected particles is represented by an exponential cutoff power law spectrum: $\dv{N}{E} \propto E^{-\Gamma}\exp\qty[E/E_c]$.}
	\centering
	\begin{tabular}{c|cccccccc}
		\hline
    	Accelerator & \multicolumn{8}{c}{\rule{2cm}{0.5pt} Hadronic \rule{2cm}{0.5pt}}\\
		 LS\,5039 & Object & $n_H$ ($\centimeterminusthree$) & $W$ or $\dot{W}$ & & $\Gamma$ & $E_C$ ($\TeV$) & $W_\text{SNR}$\footnote{5} or $\dot{W}_\text{total}$\footnote{6} & \\
		 \hline
		 Impulsive (SNR) & A & $7.0$ & $8.0\times10^{49}$ & $\ergs$ & $2.0$ & $50$ & $3.9\times10^{51}$ & $\ergs$ \\
		 $t=1\times 10^3~\si{yrs}$ & B & $79.8$ & $6.0\times10^{48}$ & & $2.0$ & $50$ & $1.5\times10^{50}$ \\
		 & C & $3.6$ & $1.0\times10^{50}$ & & $2.0$ & $50$ & $4.9\times10^{51}$  \\
		 \hline
		 Impulsive (SNR) & A & $7.0$ & $1.0\times10^{50}$ & $\ergs$ & $2.0$ & $50$ & $4.9\times10^{51}$ & $\ergs$ \\
		 $t=1\times 10^5~\si{yrs}$ & B & $79.8$ & $8.0\times10^{48}$ & & $2.0$ & $50$ & $2.0\times10^{50}$ \\
		 & C & $3.6$ & $1.5\times10^{50}$ & & $2.0$ & $50$ & $7.4\times10^{51}$ \\
		 \hline
		 Impulsive (SNR) & A & $7.0$ & $3.0\times10^{51}$ & $\ergs$ & $1.0$ & $50$ & $1.5\times10^{53}$ & $\ergs$ \\
		 $t=1\times 10^6~\si{yrs}$ & B & $79.8$ & $4.0\times10^{49}$ & & $1.5$ & $50$ & $1.0\times10^{51}$ \\
		 & C & $3.6$ & $4.0\times10^{51}$ & & $1.0$ & $50$ & $2.0\times10^{53}$ \\
		 \hline
		Continuous (accretion) & A & $7.0$ & $2.3\times10^{39}$ & $\ergspersecond$ & $2.0$ & $50$ \\
		$t=1\times 10^3~\si{yrs}$ & B & $79.8$ & $2.0\times10^{38}$ & & $2.0$  & $50$ & $7.0\times 10^{39}$ & $\ergspersecond$ \\
		 & C & $3.6$ & $4.5\times10^{39}$ & & $2.0$ & $50$ \\
		\hline
		Continuous (accretion) & A & $7.0$ & $2.8\times10^{37}$ & $\ergspersecond$ & $2.0$ & $50$ \\
		$t=1\times 10^5~\si{yrs}$ & B & $79.8$ & $2.0\times10^{36}$ & & $2.0$ & $50$ & $7.0\times 10^{37}$ & $\ergspersecond$ \\ 
		 & C & $3.6$ & $4.0\times10^{37}$ & & $2.0$ & $50$ \\
		\hline
		Continuous (accretion) & A & $7.0$ & $2.5\times10^{36}$ & $\ergspersecond$ & $2.0$ & $50$ \\
		$t=1\times 10^6~\si{yrs}$ & B & $79.8$ & $3.5\times10^{35}$ & & $2.0$ & $50$ & $6.9\times 10^{36}$ & $\ergspersecond$ \\
		 & C & $3.6$ & $4.0\times10^{36}$ & & $2.0$ & $50$ \\
		\hline
		\hline
		Accelerator & \multicolumn{8}{c}{\rule{2cm}{0.5pt} Leptonic \rule{2cm}{0.5pt}}\\
		LS\,5039 & Object & $n_H$ ($\centimeterminusthree$) & $W$ or $\dot{W}$ & & $\Gamma$ & $E_C$ ($\TeV$) & $W_\text{SNR}$ or $\dot{W}_\text{total}$ \\
		 \hline
		 Impulsive (SNR) & A & $7.0$ & $4.0\times10^{48}$ & $\ergs$ & $2.0$ & $10$ & $2.0\times10^{50}$ & $\ergs$ \\
		 $t=1\times 10^3~\si{yrs}$ & B & $79.8$ & $2.5\times10^{48}$ & & $2.0$ & $10$ & $6.4\times10^{49}$ \\
		 & C & $3.6$ & $3.0\times10^{48}$ & & $2.0$ & $10$ & $1.5\times10^{50}$ \\
		 \hline
		 Impulsive (SNR) & A & $7.0$ & $5.0\times10^{48}$ & $\ergs$ & $1.7$ & $50$ & $2.5\times10^{50}$ & $\ergs$ \\
		 $t=1\times 10^5~\si{yrs}$ & B & $79.8$ & $2.0\times10^{49}$ & & $1.0$ & $10$ & $5.1\times10^{50}$ \\
		 & C & $3.6$ & $5.0\times10^{48}$ & & $2.0$ & $10$ & $2.5\times10^{50}$ \\
		 \hline
		 Impulsive (SNR) & A & $7.0$ & $3.0\times10^{50}$ & $\ergs$ & $1.7$ & $100$ & $1.5\times10^{52}$ & $\ergs$ \\
		 $t=1\times 10^6~\si{yrs}$ & B & $79.8$ & & & & \\
		 & C & $3.6$ & $2.0\times10^{50}$ & & $2.0$ & $10$ & $9.9\times10^{51}$ \\
		 \hline
		Continuous (accretion) & A & $7.0$ & $1.0\times10^{38}$ & $\ergspersecond$ & $2.0$ & $10$ \\
		$t=1\times 10^3~\si{yrs}$ & B & $79.8$ & $8.5\times10^{37}$ & & $2.0$ & $10$ & $6.9\times 10^{38}$ & $\ergspersecond$ \\
		 & C & $3.6$ & $5.0\times10^{38}$ & & $2.0$ & $10$ \\
		\hline
		Continuous (accretion) & A & $7.0$ & $3.5\times10^{35}$ & $\ergspersecond$ & $1.7$ & $10$ \\
		$t=1\times 10^5~\si{yrs}$ & B & $79.8$ & $9.0\times10^{35}$ & & $2.0$ & $10$ & $1.5\times 10^{36}$ & $\ergspersecond$ \\
		 & C & $3.6$ & $2.0\times10^{35}$ & & $1.5$ & $10$ \\
		\hline
		Continuous (accretion) & \textbf{A} & $\boldsymbol{7.0}$ & $\boldsymbol{2.0\times10^{35}}$ & $\ergspersecond$ & $\boldsymbol{1.7}$ & $\boldsymbol{10}$ \\
		$\boldsymbol{t=1\times 10^6~\si{yrs}}$ & \textbf{B} & $\boldsymbol{79.8}$ & $\boldsymbol{7.5\times10^{35}}$ & & $\boldsymbol{1.8}$ & $\boldsymbol{30}$ & $\boldsymbol{1.0\times 10^{36}}$ & $\ergspersecond$ \\
		 & \textbf{C} & $\boldsymbol{3.6}$ & $\boldsymbol{9.0\times10^{34}}$ & & $\boldsymbol{1.5}$ & $\boldsymbol{10}$ \\
		\hline
% 		Continuous (accretion) & A & $7.0$ & $2.0\times10^{35}$ & $\ergspersecond$ & $1.7$ & $10$ \\
% 		$t=1\times 10^6~\si{yrs}$ & B & $79.8$ & $7.5\times10^{35}$ & & $1.8$ & $30$ & $1.0\times 10^{36}$ & $\ergspersecond$ \\
% 		 & C & $3.6$ & $9.0\times10^{34}$ & & $1.5$ & $10$ \\
% 		\hline
	\end{tabular}
	\begin{tablenotes}
	\item \footnotemark[5]{${W}_\text{SNR}$: Inferred energy budget of high energy particles inside progenitor SNR related to LS\,5039}
	\item \footnotemark[6]{$\dot{W}_\text{total}$: The total injection luminosity of all three clouds}
	\item Plausible scenarios are shown in bold
	\item Matching scenarios have have systematic variation of up to $56\%$ in energy budget $W$ or luminosity $\dot{W}$, $12\%$ in the spectral index $\Gamma$ and $12\%$ in the cutoff energy $E_c$ (see text and figure \ref{fig:example_SED})
	\end{tablenotes}
	\label{tab:SED_sum_5039}
	\end{threeparttable}
\end{table*}

==> removed.tex <==
% \begin{figure}
% 	\includegraphics[width=\columnwidth]{Yama_Spectrum.pdf}
%     \caption{Integrated Energy Spectrum from the region south of HESS J1825-137 as calculated by the \fermi LAT team \citep{Araya:2019dez}. The green line represents the best fit to a power law. Included is the spectral points measured by HESS towards HESS J1825-137 \citep{Aharonian:2005kj}}
%     \label{fig:Yama_Spectrum}
% \end{figure}
